Coded Caching for Heterogeneous Wireless Networks

This chapter provides an overview of coded caching in the context of heterogeneous wireless networks. We begin by briefly describing the key idea behind coded caching and then discuss in detail the impact of various aspects such as non-uniform content popularity, multiple cache access, and interference.

==> coded/sections/multi-access-bkup.tex <==

So far, we have only considered situations in which each user accesses exactly one cache, with no flexibility.
However, in a wireless heterogeneous network such as the one in \figurename~\ref{coded:fig:hetnet}, the density of access points that have caches could be high enough for each user to potentially access a large number of caches.
This enables some interesting capabilities that can be harnessed to achieve a lower broadcast rate $R$ for the same cache memory $M$.
For instance, each user could have access to the contents of multiple caches at once, effectively increasing the memory available to it.
Alternatively, we could allow the system to adaptively assign to each user one cache out of a set of nearby caches, based on the file that it requested.
In this section, we explore the latter approach in detail as studied in \cite{HKMDadaptive}, and leave the former as a short discussion at the end.

\subsection{Overview of Adaptive User-to-Cache Matching}

In the adaptive matching setup, we keep the restriction of each user accessing the contents of exactly one cache, but allow the flexibility of choosing which cache (possibly among some subset of caches) the user should access based on its requested file.
Such a problem was studied in \cite{leconte2012, moharir2016}, in the extreme case where all users are able to access any cache.
An additional restriction is a load constraint on the caches: each cache can only serve at most one user.
The surprising insight in both papers is that, contrary to the ``static matching case'' where each user is pre-attached to a unique cache (the setting described in Section~\ref{coded:sec:overview}), an approximately-optimal scheme is to replicate complete files across multiple caches in proportion to their popularity in the placement phase;, and then during the delivery phase, match as many users as possible to a cache that holds its requested file. 


We thus observe a dichotomy between two extremes: in the static matching case (when each user is restricted to one cache), appropriate splitting of files and careful placement of subfiles to enable coded-multicast transmissions during delivery as described in Section~\ref{coded:sec:overview} is approximately optimal, while simple file replication is not; on the other hand, in the fully ``adaptive matching case" where each user can be matched to any cache during the delivery phase, appropriate file replication coupled with maximum matching during delivery is approximately optimal, while a static pairing of users and caches along with the coded caching approach of Section~\ref{coded:sec:overview} is sub-optimal.
The natural next question is then: what happens when each user can be matched adaptively to one of a \emph{subset} of caches?
This problem was studied in \cite{HKMDadaptive}, and we will discuss its main results here.

\subsection{System Model}
\label{Sec:sysmodeladapmat}
\begin{figure}
\centering
\includegraphics[scale=\codedsetupfigsscale]{setup-adaptive.pdf}
\caption{Partial adaptive matching setup.
The caches are partitioned into clusters, and each user can be matched to one cache in its cluster, with a load constraint on the caches.
Excess users in a cluster cannot be matched, such as the user colored in grey.}
\label{coded:fig:adaptive-setup}
\end{figure}

Suppose there is a content library of $N$ files, called $W_1,\ldots,W_N$.
There are $K$ caches, partitioned into $K/d$ mutually exclusive \emph{clusters} of $d$ caches each (assume $d$ divides $K$).
At each cluster $c$, there is a stochastic number of users $u_n(c)$ that request file $W_n$, where $u_n(c)$ is a Poisson random variable of parameter $\rho d/N$, with $\rho\in(0,1/2)$ a constant.
Thus at every cluster (whose size is $d$ caches), the expected number of users is $\rho d$.
We will refer to $\mathbf{u}=\{u_n(c)\}_{n,c}$ as the \emph{user profile}.

In addition to the usual placement and delivery phases, there is an intermediate \emph{matching phase}, which occurs after the users have made their requests.
In this phase, we assign each user in a cluster to one cache in the same cluster, subject to a load constraint of no more than one user per cache.
Thus if there are more users than caches in a cluster ($\sum_n u_n(c)>d$ for some $c$), there will necessarily be some unmatched users who will have access to the contents of no cache.
Note that the placement phase occurs without knowing the user profile, while both the matching phase and the delivery phase have of knowledge of the user profile.

Let $R_\mathbf{u}$ denote the broadcast rate given a specific user profile $\mathbf{u}$.
We are interested in the expected rate $\bar R = \mathbb{E}_\mathbf{u}[R_\mathbf{u}]$, and more specifically  the optimal expected rate $\bar R^\star(M)$ for every memory $M$ over all possible placement, matching, and delivery strategies.

The choice of a Poisson number of users is useful as it not only more closely models real-world user requests, but also simplifies the analysis in this problem.
There is also little difference, fundamentally, between the Poisson model and the model with a fixed number of users (such as the one studied in the previous sections), as long as the cluster size $d$ is large enough, namely $d=\Omega(\log K)$.
This means that comparisons with other works in the literature are possible.
Note that for smaller $d$, the Poisson model is less meaningful; when $d=1$ for instance, there is positive probability for each cluster to have more than one user, which means that with high probability, a significant fraction of the users cannot be matched to any cache and resultantly a high server transmission rate is necessary irrespective of the cache memory size.

As mentioned above, the Poisson model only makes sense for $d=\Omega(\log K)$, and so we adopt this regularity condition in this section.
More precisely, we assume that
\begin{equation}
\label{coded:eq:d-ge-logk}
d \ge \frac{2(1+t_0)}{\alpha} \log K,
\end{equation}
where $\alpha=-\log(2\rho e^{1-2\rho})>0$, and $t_0>0$ is some constant.
Finally, we restrict our attention to the case when $N\ge K$.


\subsection{Balancing Two Extremes}

The model described above, known as the partial adaptive matching setup, is a generalization of the two extremes.
When $d=1$, we have a static matching setup as in \cite{maddah-ali2012} (while the Poisson model is not meaningful here, insights can still be gained).
When $d=K$, we have the full adaptive matching setup as in \cite{leconte2012, moharir2016}.

As discussed above, there is a dichotomy between these two extremes: the former favors a coded delivery scheme, while the other favors an uncoded replication scheme.
In what follows, we examine how each scheme performs if adapted to the partial adaptive matching setup.
Specifically, we look at:
\begin{itemize}
\item Pure Coded Delivery (PCD): ignores any potential adaptive matching benefits by arbitrarily assigning users to caches, and applying a standard Maddah-Ali--Niesen scheme as discussed in Section~\ref{coded:sec:overview};
\item Pure Adaptive Matching (PAM): ignores any potential coding gains and focuses only on file replication within a cluster and on adaptively matching users to caches within a cluster.
\end{itemize}

As we will see, in the general case we observe two regimes, and each scheme will be preferred in one regime.
These regimes are roughly defined by a threshold on the \emph{total cluster memory} $dM$: when $dM\ll N$ then PCD is favorable, and when $dM\gg N$ then PAM is favorable.
Furthermore, in each regime, the favorable scheme is approximately optimal for almost all values of the cache memory.
This is illustrated in \figurename~\ref{coded:fig:pam-pcd}.
Notice that in the special case $d=1$ (respectively, $d=K$), \figurename~\ref{coded:fig:pam-pcd} shows that PCD (respectively, PAM) is always preferred, as expected from the previous results.

\begin{figure}
\centering
\includegraphics[width=.5\textwidth]{pam-pcd-graph.pdf}
\caption{An approximate visualization of the regimes in which each scheme is more favorable.
The boundary between the PCD- and PAM-dominated regions is blurry: the regime $\Omega(N)<dM<O(N\log N)$ is still not very well understood.}
\label{coded:fig:pam-pcd}
\end{figure}

Each of the two schemes focuses on one idea: PCD ignores adaptive matching in favor of coding gains, and PAM ignores coded delivery in favor of adaptive matching gains.
A hybrid coding and matching (HCM) scheme is introduced in \cite{HKMDadaptive} which performs better than both schemes in most memory regimes.


\subsection{The Pure Coded Delivery (PCD) scheme}

The PCD scheme is a straightforward adaptation of the Maddah-Ali--Niesen scheme described in Section~\ref{coded:sec:overview}; the placement phase is identical to the one  described there. 
During the matching phase, we pick any valid user-to-cache matching and provide each user with access to the corresponding cache; this is sufficient since the placement is completely symmetric with respect to the caches and the files. The delivery phase is conducted in two parts:
\begin{enumerate}
\item For the subset of users which were matched to caches, delivery proceeds in the same fashion as in Section~\ref{coded:sec:overview} by creating coded-multicast transmissions.
\item Any users that were not matched (because there are more users than caches in their cluster) will simply be served directly by the server. 
\end{enumerate}

Note that for the model described in Section~\ref{Sec:sysmodeladapmat}, the expected number of such unmatched users is very small.
In fact it can be shown that
\[
\mathbb{E}[U^0] \le K^{-t_0}/\sqrt{2\pi},
\]
where $U^0$ is the total number of excess users across all clusters. Note that the expected number of excess users goes to zero as $K$ increases. All the other users (i.e., those that are matched to some cache) will be served by the basic Maddah-Ali--Niesen scheme, and so PCD can achieve the rate in the following theorem.

\begin{theorem}
\label{thm:pcdrate}
For the partial adaptive matching model described in Section~\ref{Sec:sysmodeladapmat}, the expected rate achieved by PCD is
\[
\bar R^\mathrm{PCD}(M) \le \min\left\{ \rho d, \left[\frac{N}{M} - 1\right]^+ + \frac{K^{-t_0}}{\sqrt{2\pi}} \right\}.
\]
\end{theorem}

Notice that this is not much different to the rate achieved in the static matching setup.
This is expected since we are not making any intelligent use of the adaptive matching feature at all in PCD. However, this turns out to be approximately optimal when the total  memory in any  cluster is not enough to hold the entire library, as stated next.

\begin{theorem}
\label{thm:PCDopt}
When $M\le(1-e^{-1}/2)N/2d$, the expected rate achieved by PCD is approximately optimal in the sense that
\[
\bar R^\mathrm{PCD}(M) \le C \cdot \bar R^\star(M) + o(1),
\]
where $R^\star(M)$ is the information-theoretically optimal rate, $C$ is a constant independent of the problem parameters, and the $o(\cdot)$ notation is to be understood with respect to the growth of $K$.
\end{theorem}

We skip the proof of these results here and instead point the interested reader to  \cite{HKMDadaptive}, which has all the details as well as discusses more general scenarios with non-uniform content popularity.


\subsection{The Pure Adaptive Matching (PAM) scheme}

As previously mentioned, the PAM scheme takes the opposite approach to PCD.
It ignores all possible coding in favor of a more intelligent matching of users to caches.
The idea is to store only replicas of files in every cluster, and rely as much as possible on the matching phase to match each user to a cache that contains the file that it requested.

More precisely, the three phases work as follows.
In the placement phase, if the total cluster memory is $dM$, then we store a complete copy of every file in $\lfloor dM/N\rfloor$ caches in every cluster.
In the matching phase, we find the best matching of users to caches so that the number of users matched to a cache containing their requested file is maximized.
In the delivery phase, any users that could not be successfully matched to a suitable cache are served directly from the server.

Notice that the scheme only really takes off once $dM\ge N$: for smaller memory values, there is a significant fraction of users who remain unmatched and have to be served directly by the server.
What's more interesting is that after this threshold of $dM\ge N$ the achieved expected rate decays exponentially with the cluster memory!
The precise rate expression is given in the following theorem.

\begin{theorem}
For the partial adaptive matching model described in Section~\ref{Sec:sysmodeladapmat},  the expected rate achieved by PAM is
\[
\bar R^\mathrm{PAM}(M) \le \begin{cases}
\rho K & \text{if $M<N/d$;}\\
KMe^{-\rho h dM/N} & \text{if $M\ge N/d$,}
\end{cases}
\]
where $h=(1/\rho)\log(1/\rho)+1-1/\rho$.
\end{theorem}

The proof follows along similar lines as \cite{leconte2012}, which focuses on the fully adaptive matching case, and generalizes the results to the partially adaptive matching case.

Notice that $\bar R^\mathrm{PAM}(M)=o(1)$ when $dM>\Omega(N\log N)$. Thus, once the total cluster memory is slightly larger than the total catalogue size, the PAM scheme requires negligible server transmission rate. This also trivially implies that PAM is approximately information-theoretically optimal in that regime.
Combining with Theorem~\ref{thm:PCDopt}, we have that PCD is approximately optimal when $dM<O(N)$ and PAM is approximately optimal when $dM>\Omega(N\log N)$, as illustrated approximately (ignoring the $\log N$ factor for simplicity) in \figurename~\ref{coded:fig:pam-pcd}.


\subsection{The Hybrid Coding and Matching (HCM) scheme}

So far, we have looked at two schemes that each focuses on a single gain: either a coding gain or an adaptive matching gain.
The schemes are approximately optimal in complementary regimes, as illustrated in \figurename~\ref{coded:fig:pam-pcd}.
This section explores a hybrid scheme that unifies coded delivery and adaptive matching by incorporating ideas of both PCD and PAM.
This Hybrid Coding and Matching (HCM) scheme, first introduced in \cite{HKMDadaptive}, turns out to perform better than both PCD and PAM in most memory regimes.

The hybrid scheme combines ideas from both PCD and PAM by introducing a coloring scheme at both the cache level and the file level.
First, we choose a certain number of colors $\chi\in\{1,\ldots,d\}$.
The exact value is not important for now; the ideas work for any $\chi$.
We then partition the caches in every cluster into $\chi$ subsets of (almost) equal size, and color each subset with a unique color.
Similarly, we partition the files in the content library into $\chi$ subsets of (almost) equal size, and color each subset with one color.
Finally, we apply the coded delivery ideas \emph{within each color}, while applying the adaptive matching ideas \emph{across colors}.

More precisely, the three phases proceed as follows.
In the placement phase, for every color $x$ we perform a Maddah-Ali--Niesen placement of the files \emph{of color $x$} in only the caches of the same color.
The placement phase is agnostic to the cluster to which a cache belongs.
In the matching phase, every user can be matched to an arbitrary cache whose color matches the file that the user requested; the user is matched to the color, but the choice of cache within that color is arbitrary.
Naturally, the matching is limited to a cache within the user's cluster.
In the delivery phase, the Maddah-Ali--Niesen coded delivery is performed for every color $x$ separately, and unmatched users are served directly.
Like the placement phase, the delivery phase ignores clusters and serves all users of the same color in the same broadcast message.

Since we have $\chi$ sub-systems of $N/\chi$ files, each running a separate Maddah-Ali--Niesen scheme, using Theorem~\ref{thm:pcdrate} we can show that the hybrid scheme can achieve a rate of
\[
\bar R(M) \approx \min\left\{ \rho K, \chi \cdot \left( \frac{N/\chi}{M} - 1 \right) + \bar U^0(\chi) \right\},
\]
where $\bar U^0(\chi)$ is the expected number of unmatched users when choosing $\chi$ colors.
What is left is therefore to choose the right value of $\chi$.

If the number of colors is too small, then there is little benefit in adaptive matching since the number of choices is reduced.
Conversely, if the number of colors is too large, then the number of caches in each color becomes small, and it becomes likely that a significant number of colors have fewer caches than there are users requesting a file from them; the number of unmatched users thus becomes too large.
The balance is struck when $\chi\approx d/\log K$ colors, as stated more precisely in the next theorem.

\begin{theorem}
For any $t\in[0,t_0]$, the HCM scheme can achieve an expected rate of
\[
\bar R^\mathrm{HCM}(M) \le \begin{cases}
\min\left\{ \rho K, \frac{N}{M} - \chi + \frac{K^{-t}}{\sqrt{2\pi}} \right\} & \text{if $M\le\lfloor N/\chi\rfloor$;}\\
\frac{K^{-t}}{\sqrt{2\pi}} & \text{if $M\ge\lceil N/\chi\rceil$,}
\end{cases}
\]
where $\chi = \lfloor \alpha d/(2(1+t)\log K)\rfloor$.
\end{theorem}

The rate expression can be approximately written as
\[
\bar R^\mathrm{HCM}(M) \approx \min\left\{ \rho K,
\left[ \frac{N}{M} - \Theta\left(\frac{d}{\log K}\right) \right]^+
+ o(1) \right\}.
\]

Comparing the performances of PCD, PAM, and HCM, we find that HCM performs better than both of them in most memory regimes.
In fact, HCM is a unified scheme that is approximately optimal for almost all memory regimes.
Specifically, we have:
\begin{itemize}
\item For all $M\ge0$, HCM performs better than PCD;
\item When $dM\le O(N)$, both HCM and PCD are approximately optimal, while PAM is not;
\item When $dM\ge\Omega(N\log K)$, both HCM and PAM are trivially approximately optimal and achieve a rate of $o(1)$, while PCD is not;
\item The intermediate regime $\Omega(N)\le dM\le O(N\log K)$ is not very well understood and the exact relationship between the different rates, as well as their approximate optimality, is not known.
\end{itemize}
More details can be found in \cite{HKMDadaptive}.

\subsection{Simultaneous Cache Multi-Access}
\input{coded/sections/simultaneous-access.tex}



==> coded/sections/popularity-bkup.tex <==
By studying the worst-case rate over all possible user demands, the problem in \cite{maddah-ali2012} effectively ignores any content popularity, since in practice some files can be requested more frequently than others.
One way to incorporate content popularity into the problem is by setting the user requests to be stochastic, following some probability distribution, and then analyzing the expected broadcast rate.
A common distribution to model content popularity is the Zipf distribution, which is widely observed for many content libraries such as the YouTube video catalogue \cite{YoutubeRepository}.
Coded caching is studied under such a distribution in \cite{JiZipf}, and the approximately optimal expected server transmission rate is characterized.
In \cite{niesen2017coded, ZhangArbitrary}, the case of arbitrary popularity distributions is studied and the approximately optimal expected rate is derived.
%A surprising result is that the optimal expected rate can be approximately achieved by dividing the files into only

In general, the popularity of a file can be thought of as the likelihood that a given user will request this file.
Under a stochastic popularity model, this translates to a probability distribution over the files such that each user requests one file based on this probability.
Note that, since the number of files is typically large compared to the number of users, we cannot reliably predict the number of users requesting each file from prior requests, especially for the less popular files.
However, if the files are partitioned into a small number of levels by grouping together contents of similar popularity, we can more reliably estimate the cumulative popularity across these levels. If the number of users is large compared to the number of levels, the number of users \emph{per level} under the stochastic popularity model will concentrate around the average value. The multi-level popularity model, introduced in \cite{HKDmultilevel}, captures this aspect by making the number of users requesting files from each level to be fixed, deterministic, and known \emph{a priori}; the worst-case rate (under this restriction on the demand vectors) is then analyzed in a similar vein as in Section~\ref{sec:setupbasic}. We discuss this multi-level popularity model in this section. 

%Another approach to model content popularity is the multi-level model, which partitions files into a few popularity levels. In this model, introduced in \cite{HKDmultilevel}, the number of users requesting files from each level is fixed; the worst-case rate (under this restriction on the demand vectors) is then analyzed in a similar vein as in Section~\ref{sec:setupbasic}.
%The multi-level popularity model is useful for several reasons.
%First, it is much more practical to estimate the popularity of a group of files than that of just a single file.
%Second, even under the stochastic approach, coded caching benefits can only be obtained when some files are grouped together and treated as though they are equally popular.
%Thus this model can faithfully focus on the non-uniform popularity aspect without the added complexity of a probabilistic analysis.
%We discuss multi-level popularity in Section~\ref{coded:sec:popularity}.


%One of the most important aspects of content distribution is leveraging the non-uniformity of content popularity.
%As discussed in Section~\ref{coded:sec:overview:popularity}, there are several ways to model this non-uniformity, and we here adopt the multi-level model introduced in \cite{HKDmultilevel}.

%In general, the popularity of a file can be thought of as the likelihood that a given user will request this file.
%Under a stochastic popularity model, this translates to a probability distribution over the files such that each user requests one file based on this probability.
%Note that, since the number of files is typically large compared to the number of users, we cannot reliably predict the number of users requesting each file from prior requests, especially for the less popular files.
%However, if the files are partitioned into a small number of levels by grouping together contents of similar popularity, we can more reliably estimate the cumulative popularity across these groups. If the number of users is large compared to the number of groups, the number of users \emph{per group} under the stochastic popularity model will concentrate around the average value. The multi-level popularity model captures this aspect by making the number of users per group to be fixed, deterministic, and known \emph{a priori}.

More formally, in the multi-level popularity model, the files in the content library are partitioned into a certain number of groups called popularity levels.
Each level $i\in\{1,\ldots,L\}$ consists of $N_i$ files, and there are a total of $K_i$ users requesting files from this level.
Each of these $K_i$ users can request any file belonging to level $i$.
It is useful to think of the popularity of each file in level $i$ as being proportional to the number of users per file of the level, $K_i/N_i$.
For simplicity, we restrict the discussion here to the case where there are more files than users per for every level, i.e., $N_i\ge K_i$ for all $i\in\{1,\ldots,L\}$. Note that the setup studied in Section~\ref{coded:sec:overview} is a special case with $L =1$ level, $N_1 = N$, and $K_1 = K$.  

The multi-level popularity model turns out to be useful in studying how the total number of users in the network, as compared to the number of caches, affects the system under non-uniform popularity.
We will look at two extremes: one in which each cache has exactly one associated user (the single-user setup), and one in which each cache has a large number of associated users (the multi-user setup).
In the single-user setup, only one level is represented at each cache since each user requests one file from one popularity level, as shown in \figurename~\ref{coded:fig:setup-ml-su}.
In the multi-user setup, the number of users is large enough for every level to be represented at every cache by at least one user, as shown in \figurename~\ref{coded:fig:setup-ml-mu}.
Interestingly, it turns out that the strategies required for these two setups are quite different: a level-merging approach works for the single-user setup, while a level-separation approach works for the multi-level setup.

\begin{figure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[scale=\codedsetupfigsscale]{setup-ml-su.pdf}
\caption{The single-user setup.}
\label{coded:fig:setup-ml-su}
\end{subfigure}

\begin{subfigure}{\textwidth}
\centering
\includegraphics[scale=\codedsetupfigsscale]{setup-ml-mu.pdf}
\caption{The multi-user setup.}
\label{coded:fig:setup-ml-mu}
\end{subfigure}
\caption{Multi-level popularity, with $L=2$ levels.}
\end{figure}

In order to understand the major difference between these two setups, it is useful to first reflect on what enables the coding gains in the original setup in Section~\ref{coded:sec:overview}.
Recall that a coded message from the server consists of a linear combination of parts of files requested by a subset of users, for example see \eqref{Eqn:transmittedmsg}. 
Each such user has access to \emph{different} side-information through their distinct caches. 
It is precisely this difference in side-information that allows the same linear combination to be beneficial to multiple users possibly requesting distinct files.
If two users' cache contents were identical, then their side-information is identical and no coding gains can be achieved among them.
%Let us call this the \emph{side-information principle}.

Moreover, because of the symmetry of the delivery message in \eqref{Eqn:transmittedmsg}, the procedure is most efficient when the involved subfiles are of the same size; or equivalently when the files involved are stored equally in each cache. When adapting this to the non-uniform popularities setup, this creates a conflict: since the more popular files are more likely to be requested, we would want to give them a larger portion of the cache memory than the less popular files. However, as mentioned before, this would negatively impact the efficiency of coded messages involving requests for files with significantly different popularities. Hence there is potentially a dilemma between giving the more popular files a larger memory share on the one hand, and obtaining more efficient coding opportunities on the other hand.

The dilemma is naturally resolved for the multi-user setup. Notice from  \figurename~\ref{coded:fig:setup-ml-mu} that the users can be partitioned into ``rows'' of $K$ users each, such that each user in the row connects to one cache and requests a file from the same popularity  level. A natural strategy here is to ensure that each linear combination the server sends is intended only for a subset of users belonging to the same row. Since all involved requests in a row will be for files belonging to the same level, they will have the same popularity and hence the same allocated cache memory.  Furthermore, grouping an additional  user (requesting a distinct file) with a row of $K$ users in a single coded-multicast transmission cannot be beneficial since this user will necessarily share a cache with another user in the considered row and thus have access to the same side-information, and hence as discussed before no coding gains can be obtained between them.
As we will see later, the approximately optimal strategy here is to partition each cache amongst the various levels during the placement phase and then address the demands in each row of users separately during the delivery phase using coded-multicast transmissions as discussed in Section~\ref{coded:sec:overview}. 
%


On the other hand, the dilemma is not so easily resolved in the single-user setup. Notice from \figurename~\ref{coded:fig:setup-ml-su} that in this case there is only one ``row'' of users in which all the file popularity levels are represented. This is unlike the multi-user setup where all users in a row requested files from the same popularity level, and hence if we allow all linear combinations in the server transmission, we might have to combine requests for files with very different popularities. On the other hand, if we restrict server transmissions to combine only requests belonging to the same popularity level, that will limit the coded-multicasting opportunities severely and increase the required server transmission rate. As we will see later, it turns out that the approximately optimal strategy here is to ``merge'' a subset of the higher popularity levels so that all the files belonging to them are given the same amount of memory, and so that the requests belonging to these levels can be efficiently combined in the coded-multicast messages. 

Thus, the schemes corresponding to the multi-user and single-user setups have different philosophies and this difference marks the dichotomy between the two setups. Next, we study each of these setups in more detail.


\subsection{The Single-User Setup}

In the single-user setup, there is exactly one user connected to each of the $K$ caches. As mentioned before, $K_i$ users  in the system request  a file from level $i$ and $K_1+\cdots+K_L=K$. Importantly, while placing content in the caches, we know exactly how many users will request a file from each level, but we do not know \emph{which} users will request from which level.

As discussed before, the idea in this setup is to strike a balance between two opposing principles: creating coding opportunities across popularity levels on the one hand, and allocating more of the cache memory to the more popular files on the other hand.
The balance that turns out to be approximately optimal is to group the levels into two groups, which we will call $H$ and $I$.
The files belonging to levels in the set $I$ will all be treated as if they are of the same popularity and are all allocated the same amount of memory; effectively the levels in $I$ are merged into one super-level with $\sum_{i\in I}N_i$ files and $\sum_{i\in I}K_i$ users.
All the cache memory will be given to the set $I$, while the files in set $H$ will not be stored at all.
A coded caching scheme is then used on the set $I$ as described in Section~\ref{sec:centscheme}, and all requests for files from set $H$ are handled by direct unicast transmissions from the server.

We can therefore apply Theorem~\ref{coded:thm:singlelevel-achieve} on each of $H$ and $I$ separately, which using \eqref{coded:eq:singlelevel-ub} yields an achievable rate upper-bounded by
\begin{equation}
\label{Eqn:AchievableRateSingleUserPerCache}
R_\mathrm{SU}(M) \le \max\left\{\frac{\sum_{i\in I}N_i}{M} - 1, 0\right\} + \sum_{h\in H}K_h.
\end{equation}
The maximization with zero is necessary since depending on the choice of $I$, $M$ could be larger than $\sum_{i\in I}N_i$.

\begin{example}
Consider an example multi-level single-user setup with $L=3$ file popularity levels, $N_1 = 10$,$N_2 = 50$, $N_3 = 100$ files and $K_1 = 100$, $K_2 = 50$, $K_3 = 5$ users. Consider the memory per cache to be $M = N_1 = 10$. We evaluate the rate of the above proposed strategy for different choices of $H$, $I$:
%
\begin{enumerate}
\item \emph{Store most popular only}: In this case, we set $I = 1$ and $H = \{2,3\}$ and thus, store only the files of the most popular level, level $1$, in the caches. From \eqref{Eqn:AchievableRateSingleUserPerCache}, the rate of the scheme for this choice is $\max\{N_1 / N_1 - 1, 0\} + K_2 + K_3 = 55$. 
%
\item \emph{Treat all levels as uniform}: In this case, we set $I = \{1,2,3\}$ and $H = \phi$ and thus, allocate equal  memory to all the files. From \eqref{Eqn:AchievableRateSingleUserPerCache}, the rate of the scheme for this choice is $\max\{(N_1 + N_2 + N_3)/ N_1 - 1, 0\} = 15$.  
%
\item \emph{Merge subset of levels}: We set $I = \{1,2\}$ and $H = \{3\}$ and thus, allocate equal memory to all the files belonging to the more popular levels, levels $1$ and $2$. From \eqref{Eqn:AchievableRateSingleUserPerCache}, the rate of the scheme for this choice is $\max\{(N_1 + N_2)/ N_1 - 1, 0\} + K_3 = 10$.  
\end{enumerate}  
Thus, this example suggests that the optimal choice of $H$, $I$ is non-trivial and greatly impacts the rate of the proposed scheme. 
\end{example}
%
To understand how to choose the sets $H$ and $I$ optimally, consider the following back of the envelope calculation. Suppose that all levels except one (call it level $\ell$) have been partitioned into two sets $H'$ and $I'$.
If we put $\ell$ with $H'$, we get the achievable rate
\[
R_1(M) \approx \frac{\sum_{i\in I'}N_i}{M} + \sum_{h\in H'}K_h + K_\ell,
\]
whereas if we combine it with $I'$ we get
\[
R_2(M) \approx \frac{\sum_{i\in I'}N_i + N_\ell}{M} + \sum_{h\in H'}K_h.
\]
Then, $R_1(M)\le R_2(M)$ if and only if $K_\ell / N_\ell \le 1/M$. In this case, we choose to group level $\ell$ with $H'$. 
% on the popularity of a file to be assigned memory 
%We therefore choose to  or $I'$ based on whether $M$ is less than or greater than $N_\ell/K_\ell$.
Following this intuition, we choose the sets $H$ and $I$ as:
\begin{equation}
\label{coded:eq:singleuser-hi}
H = \left\{ h\in\{1,\ldots,L\} : K_h / N_h < 1/M\right\};\quad I = \{1,\ldots,L\} \setminus H,
\end{equation}
%
where as mentioned before, the cache memory is divided equally amongst only the files belonging to levels in $I$ in accordance with the scheme described in Section~\ref{sec:centscheme}. Recall that for our setup, we can think of the popularity of each file in level $i$ as being proportional to the number of users per file of the level, $K_i/N_i$. Thus, the above decision rule suggests $1/M$ as a popularity threshold: all files with popularity above this threshold are assigned equal memory and all files with lower popularity are not allocated any memory during the placement phase. 
 
The above scheme leads to the following achievable rate for the single-user multi-level caching setup.
\begin{theorem}
\label{thm:singleuser}
In the single-user setup, the following rate is achievable for all $L$, $K$, $\{N_i,K_i\}$, and $M$:
\[
R_\mathrm{SU}(M) \le \max\left\{ \frac{\sum_{i\in I}N_i}{M} - 1, 0 \right\} + \sum_{h\in H} K_h,
\]
where $H$ and $I$ are as defined in \eqref{coded:eq:singleuser-hi}.
\end{theorem}

As we did for the single-level setup in Section~\ref{sec:approxopt}, next we examine how the performance of the scheme proposed above compares to that of the optimal scheme. The next result  \cite{HKDmultilevel} states the approximate optimality of the achievable rate $R_{\mathrm{SU}}(M)$ in Theorem~\ref{thm:singleuser} with respect to the optimal rate $R_{\mathrm{SU}}^\star(M)$ for this setup. 
%
\begin{theorem}
\label{coded:thm:singleuser-orderoptimal}
The rate $R_\mathrm{SU}(M)$ achieved in Theorem~\ref{thm:singleuser} for the system with multi-level popularity and a single user per cache is within a constant multiplicative factor of the information-thoeretically optimal rate $R^{\star}_\mathrm{SU}(M)$. Specifically, for all values of $L$, $K$, $\{N_i,K_i\}$ with $N_i \ge K_i$, and $M$,
\[
1 \le \frac{R_\mathrm{SU}(M)}{R^\star_\mathrm{SU}(M)} \le 72.
\]
\end{theorem}
%
Note that the bound is independent of the problem parameters. As before, the proof derives information-theoretic lower bounds on the optimal rate using cut-set based arguments; details are available in  \cite{HKDmultilevel}. Finally, the focus of the above result is on proving constant factor-optimality (irrespective of system parameters) and while the factor of $72$ is very large, this can be vastly improved using the aforementioned progress made on designing better achievable strategies and lower-bound arguments.  

\subsection{Multi-User Setup}

We begin with some notation, see \figurename~\ref{coded:fig:setup-ml-mu} for an illustration of multi-level multi-user setup. For each popularity level $i$, each cache has exactly $U_i$ users requesting files from level $i$, which implies that the total number of users demanding files from level $i$ is $K_i=KU_i$. As mentioned earlier, we assume that $N_i \ge K_i=KU_i$ for each level $i$.

As compared to the single-user setup described in the previous section, the biggest difference in the multi-user setup is that every level is represented at each cache, equally across the caches.
In other words, every cache has the same user profile, where a user profile is an indicator of the number of users requesting a file from each given level. This allows separating the popularity levels and restricting all coding opportunities to be amongst users requesting files from a single level and not across levels.

More precisely, the idea is to partition the memory $M$ among the popularity levels, giving level $i\in\{1,\ldots,L\}$ a memory of $\alpha_iM$ for some $\alpha_i\in[0,1]$, and then apply the single-level coded caching scheme from Section~\ref{coded:sec:overview} on each row of users separately, with each row consisting of users requesting files from a single level.
Under this strategy, we can derive the achievable rate using Theorem~\ref{coded:thm:singlelevel-achieve} and \eqref{coded:eq:singlelevel-ub} to be
\begin{equation}
\label{eqn:multiuserachievable}
R_\mathrm{MU}(M) \le \sum_{i=1}^L U_i \cdot \min\left\{K, \max\left\{ \frac{N_i}{\alpha_iM}-1, 0 \right\} \right\}.
\end{equation}
The factor $U_i$ appears because there are exactly $U_i$ rows of users for level $i$.

By optimizing the overall rate over the memory-sharing parameters $\alpha_1,\ldots,\alpha_L$, we establish a memory allocation which we will show achieves a rate that is information-theoretically order-optimal. At a high level, this allocation is done by partitioning the popularity levels into three sets: $H$, $I$, and $J$. 
The levels in $H$ have such a small popularity that they will get no cache memory. Thus, for all levels $h\in H$, we will assign $\alpha_hM=0$.
On the opposite end of the spectrum, the most popular levels are assigned to $J$ and are given enough cache memory to completely store all their files in every cache. Thus, for every level $j\in J$, we have $\alpha_jM=N_j$, since that is the amount of memory needed to completely store all files of level $j$ in each cache. Finally, the rest of the levels, in the set $I$, will share the remaining memory among themselves, obtaining some non-zero amount of memory per cache but not enough to completely store all of their files. The more popular files should get more memory, and as discussed before we can think of $KU_i/N_i$ as representing the popularity of a level $i$.
For the order-optimal strategy we propose, we choose to give level $i$ a memory per cache of  roughly $\alpha_iM\propto N_i\cdot\sqrt{U_i/N_i}$ (hence the memory \emph{per file} is proportional to $\sqrt{U_i/N_i}$).%
\footnote{The square root comes from minimizing the rate expression in \eqref{eqn:multiuserachievable} which has an inverse function of $\{\alpha_i\}$.} 

The above assignment will represent a valid choice for the memory-sharing parameters as long as the partition $(H, I, J)$ is selected so that each $\alpha_i \in [0,1]$. When we plug the above choice of the memory-sharing parameters into \eqref{eqn:multiuserachievable}, we get the following result.
%
\begin{theorem}
\label{thm:multi-user-achievability}
Given a multi-user caching setup, with $K$ caches, $L$ levels, and, for each level $i$, $N_i$ files and $U_i$ users per cache, and a cache memory of $M$, the following rate%
\footnote{This expression of the rate is a slight approximation that we use here for simplicity as it is more intuitive.
An exact and complete description of the achievable rate can be found in \cite{HKDmultilevel}.}
is achievable:
\begin{equation}
\label{Eqn:UpperBoundMultiUserRate}
R_\mathrm{MU}(M) \approx \sum_{h\in H} KU_h
+ \frac{ \left( \sum_{i\in I} \sqrt{N_iU_i} \right)^2 }{ M - \sum_{j\in J}N_j}
- \sum_{i\in I}U_i,
\end{equation}
where $(H,I,J)$ is a partition of the set of popularity levels which satisfies:
%
\begin{IEEEeqnarray*}{lCl/rCcCl}
\forall h &\in& H, &
&& \tilde M &<& \frac1K \sqrt{\frac{N_h}{U_h}};\\
\forall i &\in& I, &
\frac1K \sqrt{\frac{N_i}{U_i}} &\le& \tilde M &\le& \left( 1+\frac1K \right)\sqrt{\frac{N_i}{U_i}};\\
\forall j &\in& J, &
\left( 1 + \frac1K \right)\sqrt{\frac{N_j}{U_j}} &<& \tilde M,
\end{IEEEeqnarray*}
where $\tilde M = (M-T_J+V_I)/S_I$, and, for any subset $A$ of the levels:
\[
S_A = \sum_{i\in A} \sqrt{N_iU_i};
\quad
T_A = \sum_{i\in A} N_i;
\quad
V_A = \sum_{i\in A} \frac{N_i}{K}.
\]
%
\end{theorem}
%
The proof of the above result is rather involved and we point the reader to \cite{HKDmultilevel} for details. Intuitively, since a level $h\in H$ receives no cache memory, all requests from its $KU_h$ users must be handled directly from the broadcast.
Since, we have $N_i\ge K_i = KU_i$ for all levels $i$, then in the worst case a total of $KU_h$ distinct files must be completely transmitted for the users requesting files from level $h$. This contributes the term $\sum_{h\in H} KU_h$ in the expression of the achievable rate \eqref{Eqn:UpperBoundMultiUserRate}. 
The users in set $J$ require no transmission as the files are completely stored in all the caches; however, it does affect the rate through the memory available for levels in $I$.
This is apparent in the expression $M-\sum_{j\in J}N_j$ in \eqref{Eqn:UpperBoundMultiUserRate}.
Finally, the levels in $I$, having received some memory, require a rate that is inversely proportional to the effective memory and that depends on the level-specific parameters $N_i$ and  $U_i$.

Finally, notice in the statement of the theorem that in the restrictions put on the class of partitions $(H,I,J)$ allowed, the different sets are largely determined by the quantity $\sqrt{N_i/U_i}$, for each level $i$ which is a function of the file popularities. Also, the conditions imposed satisfy the natural principle that the most popular levels (i.e., those with the \emph{smallest} $N_i/U_i$) will be in $J$, while the least popular levels (those with the \emph{largest} $N_i/U_i$) will go to the set $H$.

\begin{example}
Consider an example multi-level multi-user setup with $K=10$ caches, $L=3$ file popularity levels, $N_1 = 100$, $N_2 = 200$, $N_3 = 300$ files and $U_1 = 10$, $U_2 = 5$, $U_3 = 1$ users/cache. Consider the memory per cache to be $M = N_1 = 100$. We evaluate the rate of the above proposed strategy for different choices of $H$, $I$, $J$:
%
\begin{enumerate}
\item \emph{Store most popular only}: In this case, we set $J = 1$, $I = \phi$, and $H = \{2,3\}$ and thus, store only the files of the most popular level, level $1$, in the caches. From \eqref{Eqn:UpperBoundMultiUserRate}, the rate of the scheme for this choice is $KU_2 + KU_3 = 60$. 
%
\item \emph{Share memory amongst all levels}:  In this case, we set $I = \{1,2,3\}$ and thus allocate memory to each level in proportion to the square root of its popularity. From \eqref{Eqn:UpperBoundMultiUserRate}, the rate of the scheme for this choice is approximately $\frac{ \left( \sqrt{N_1U_1} + \sqrt{N_2U_2} + \sqrt{N_3U_3} \right)^2 }{ N_1 }
- (U_1 + U_2 + U_3) \approx 65 - 16 = 49$.
%
\item  \emph{Share memory amongst subset of levels}:  In this case, we set $I = \{1,2\}$ and $H=\{3\}$, and thus allocate memory only to the more popular level in proportion to the square root of its popularity. From \eqref{Eqn:UpperBoundMultiUserRate}, the rate of the scheme for this choice is approximately $KU_3 + \frac{ \left(\sqrt{N_1U_1} + \sqrt{N_2U_2} \right)^2 }{ N_1 }
- (U_1 + U_2)  = 50 - 15 = 35$.
%
%\item \emph{Treat all levels as uniform}: In this case, we allocate equal memory to all the files in the system, in effect treating them as belonging to the same popularity level with $(N_1 + N_2 + N_3)$ files with $(U_1 + U_2 + U_3)$ users per cache. From \eqref{eqn:multiuserachievable}, the rate of the scheme for this choice is $(U_1 + U_2 + U_3) \cdot \left(\frac{N_1 + N_2 + N_3}{N_1} - 1\right) = 80$.  
%
\end{enumerate}  
Thus, we say that the optimal choice of $H$, $I$, $J$ is non-trivial and greatly impacts the rate of the proposed scheme. 
\end{example}
%
The next result  \cite{HKDmultilevel} states the approximate optimality of the achievable rate $R_{\mathrm{MU}}(M)$ in Theorem~\ref{coded:thm:singlelevel-achieve} with respect to the optimal rate $R_{\mathrm{MU}}^\star(M)$. 
%
\begin{theorem}
\label{coded:thm:singleuser-orderoptimal}
The rate $R_\mathrm{MU}(M)$ achieved in Theorem~\ref{thm:multi-user-achievability} for the system with multi-level popularity and multiple users per cache is within a constant multiplicative factor of the information-thoeretically optimal rate $R^\star_\mathrm{MU}(M)$. Specifically, for all values of $L$, $K$, $M$, $\{N_i,U_i\}$ with $N_i \ge K_i$ and satisfying regularity condition\footnote{The reasoning behind this condition is that, if it did not hold for some levels $i$ and $j$, then we can think of them as essentially one level with $N_i+N_j$ files and $U_i+U_j$ users per cache.
The resulting popularity $\frac{U_i+U_j}{N_i+N_j}$ would be close to both $U_i/N_i$ and $U_j/N_j$.} $\sqrt{\frac{U_i/N_i}{U_j/N_j}} \ge \frac{1}{\beta}$,
\[
1 \le \frac{R_\mathrm{MU}(M)}{R^\star_\mathrm{MU}(M)} \le c.
\]
%
where $\beta = 198$ and $c=9909$ are constants (independent of all problem parameters).
\end{theorem}
%
Unlike the approximate optimality results presented before, the proof of this theorem requires the use of \textit{non cut-set} based arguments to derive information-theoretic lower bounds on the optimal rate; details are available in  \cite{HKDmultilevel}. As before, the constants involved can all potentially be improved greatly. 



